Efficient Floating-Point Arithmetic on Fault-Tolerant Quantum Computers

We propose a novel floating-point encoding scheme that builds on prior work involving fixed-point encodings. We encode floating-point numbers using Two's Complement fixed-point mantissas and Two's Complement integral exponents. We used our proposed approach to develop quantum algorithms for fundamental arithmetic operations, such as bit-shifting, reciprocation, multiplication, and addition. We prototyped and investigated the performance of the floating-point encoding scheme on quantum computer simulations by performing reciprocation on randomly drawn inputs and by solving first-order ordinary differential equations, while varying the number of qubits in the encoding. We observed rapid convergence to the exact solutions as we increased the number of qubits and a significant reduction in the number of ancilla qubits required for reciprocation when compared with similar approaches.

==> fig/div_box.tex <==
\begin{figure*}[tb]
    \centering
	\begin{subfigure}[t]{0.49\linewidth}
		\includegraphics[width=\linewidth]{plots/recip_error_linear.tikz}
		\caption{Relative error (linear)}
		\label{fig:div:box:linear}
	\end{subfigure}
	\begin{subfigure}[t]{0.49\linewidth}
		\includegraphics[width=\linewidth]{plots/recip_error_log.tikz}
		\caption{Relative error (log)}
		\label{fig:div:box:log}
	\end{subfigure}
	\caption{Relative error distributions of reciprocal gate output for different register widths. We characterized the error for 10-, 12-, 14-, 16-, 18-, and 20-qubit registers, with 6-, 7-, 9-, 11-, 12-, and 13-qubit mantissas, respectively, and with 4-, 5-, 5-, 5-, 6-, and 7-qubit exponents, respectively. Figs. (\protect\subref{fig:div:box:linear}) and (\protect\subref{fig:div:box:log}) show the error distributions using linear and logarithmic scales for the error, respectively. Each reciprocal gate was tested with 100 samples from a normal distribution $\mathcal{N}\Par{0,5}$ and for $L=10$ Newton iterations. We discarded samples that did not have a reciprocal that is representable after rounding, such as $0$. We treated the closest representable value at the prescribed precision of the reciprocal operation as the ground truth for error calculation.}
    \label{fig:div:box}
\end{figure*}

